An Indirect Rate-Distortion Characterization for Semantic Sources: General Model and the Case of Gaussian Observation

A new source model, which consists of an intrinsic state part and an extrinsic observation part, is proposed and its information-theoretic characterization, namely its rate-distortion function, is defined and analyzed. Such a source model is motivated by the recent surge of interest in the semantic aspect of information: the intrinsic state corresponds to the semantic feature of the source, which in general is not observable but can only be inferred from the extrinsic observation. There are two distortion measures, one between the intrinsic state and its reproduction, and the other between the extrinsic observation and its reproduction. Under a given code rate, the tradeoff between these two distortion measures is characterized by the rate-distortion function, which is solved via the indirect rate-distortion theory and is termed as the semantic rate-distortion function of the source. As an application of the general model and its analysis, the case of Gaussian extrinsic observation is studied, assuming a linear relationship between the intrinsic state and the extrinsic observation, under a quadratic distortion structure. The semantic rate-distortion function is shown to be the solution of a convex programming programming problem with respect to an error covariance matrix, and a reverse water-filling type of solution is provided when the model further satisfies a diagonalizability condition.

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}


==> subsections/gaussian-weighted.tex <==
\subsection{Results for Weighted-Average Distortion measures}
\label{u:gaussian.weighted}

\begin{theorem}
\label{thm:gaussian.weighted.achievability}
A pair $( r , \bar{D} ) \in \reals^{2}$ is an achievable rate-distortion pair for the source, distortion measures $d_{S}$, $d_{X}$ and weighted $w_{S}$, $w_{X}$ if and only if there exist a positive semi-definite matrix $\Delta$ such that
\begin{align}
    \Delta & \le \Sigma_{X} ,
    \label{e:gaussian.weighted.deltale}
\\
    \frac{1}{2}
    \log_{2} \left( \frac{\det ( \Sigma_{X} )}{\det ( \Delta )} \right)
    & \le r ,
    \label{e:gaussian.weighted.rate}
\\
    \tr ( ( w_{S} H^{T} H + w_{X} I_{m} ) \Delta )
    & \le \bar{D} - w_{S} \tr ( \Sigma_{Z} ) .
    \label{e:gaussian.weighted.trd}
\end{align}
\end{theorem}

\begin{proof}
Let $G$ denote the rate-distortion region for the source and distortion measures $d_{S}$, $d_{X}$.

Suppose that $( r , \bar{D} )$ is achievable for weights $w_{S}$, $w_{X}$. By Theorem~\ref{thm:general.relation}, there exist a $( r , D_{S} , D_{X} ) \in G$ such that $( r , \bar{D} ) = ( r , w_{S} D_{S} + w_{X} D_{X} )$. By Theorem~\ref{thm:gaussian.achievability}, there exists a positive semi-definite matrix $\Delta$ that satisfy \eqref{e:gaussian.deltale}, \eqref{e:gaussian.rate}, \eqref{e:gaussian.trds} and \eqref{e:gaussian.trdx}.
\begin{align*}
    & \tr ( ( w_{S} H^{T} H + w_{X} I_{m} ) \Delta )
    + w_{S} tr ( \Sigma_{Z} )
\\
    ={} & w_{S} \tr ( H^{T} H \Delta )
    + w_{X} \tr ( \Delta )
    + w_{S} \tr ( \Sigma_{Z} )
\\
    ={} & w_{S} [ \tr ( H \Delta H^{T} ) + \tr ( \Sigma_{Z} ) ]
    + w_{X} \tr ( \Delta )
\\
    \le{} & w_{S} D_{S} + w_{X} D_{X}
\\
    ={} & \bar{D} ,
\end{align*}
so $\Delta$ also satisfy \eqref{e:gaussian.weighted.trd}.

Conversely, suppose the existence of a positive semi-definite matrix $\Delta$ that satisfy \eqref{e:gaussian.weighted.deltale}, \eqref{e:gaussian.weighted.rate} and \eqref{e:gaussian.weighted.trd}. Define
\begin{align*}
    \delta
    & = \bar{D}
    - w_{S} \tr ( \Sigma_{Z})
    - \tr ( ( w_{S} H^{T} H + w_{X} I_{m} ) \Delta ) ,
\\
    D_{S}
    & = \tr ( H \Delta H^{T} ) + \tr ( \Sigma_{Z} ) + \delta ,
\\
    D_{X}
    & = \tr ( \Delta ) + \delta .
\end{align*}
$( r , D_{S} , D_{X} )$ is achievable because \eqref{e:gaussian.deltale}, \eqref{e:gaussian.rate}, \eqref{e:gaussian.trds} and \eqref{e:gaussian.trdx} are satisfied. We can verify $w_{S} D_{S} + w_{X} D_{X} = \bar{D}$. By Theorem~\ref{e:general.relation}, $( r , \bar{D} ) = ( r , w_{S} D_{S} + w_{X} D_{X} )$ is achievable for weights $w_{S}$, $w_{D}$.
\end{proof}

Theorem~\ref{thm:gaussian.weighted.rdf} can be verified by using Theorem~\ref{thm:gaussian.weighted.achievability} and the definition of the rate-distortion function.

\begin{theorem}
The rate-distortion function for the source, distortion measures $d_{S}$, $d_{X}$ and weights $w_{S}$, $w_{X}$ is
\begin{equation}
    R ( \bar{D} )
    = \min_{\Delta \in A ( \bar{D} )}
    \frac{1}{2}
    \log_{2} \left( \frac{\det ( \Sigma_{X} )}{\det ( \Delta )} \right)
    \label{e:gaussian.weighted.rdf}
\end{equation}
defined on $\{ \bar{D} | \bar{D} > w_{S} \tr ( \Sigma_{Z} ) \}$, where $A ( \bar{D} )$ is the set of positive semi-definite matrix $\Delta$ that satisfies \eqref{e:gaussian.weighted.deltale} and \eqref{e:gaussian.weighted.trd}.
\end{theorem}

Theorem~\ref{thm:gaussian.rdf} can be generalized to a memoryless semantic source with multiple state processes. Suppose that the distribution of an observation $X$ is $\mathcal{N} ( 0_{m} , \Sigma_{X} )$. For each $j \in \{ 0 , 1 , \cdots , k - 1 \}$, let $H_{j}$ be a $l_{j} \times m$ matrix, $Z_{j}$ be a random $l_{j}$-vector with covariance matrix $\Sigma_{j}$, and $S_{j} = H_{j} X_{j} + Z_{j}$ be a state. $X$, $Z_{0}$, $Z_{1}$, $\cdots$, $Z_{k - 1}$ are assumed to be independent. The rate-distortion function for this source and squared-error distortion measures $d_{0}$, $d_{1}$, $\cdots$, $d_{k - 1}$, $d_{X}$ is
\begin{equation*}
    R ( D_{0} , D_{1} , \cdots , D_{k - 1} , D_{X} )
    = \min
    \frac{1}{2}
    \log_{2} \left( \frac{\det ( \Sigma_{X} )}{\det ( \Delta )} \right)
\end{equation*}
defined on $\{ ( D_{0} , D_{1} , \cdots , D_{k - 1} , D_{X} ) | D_{0} > \tr ( \Sigma_{0} ) , D_{1} > \tr ( \Sigma_{1} ) , \cdots , D_{k - 1} > \tr ( \Sigma_{k - 1} ) , D_{X} > 0 \}$. The constraints of the minimization are
\begin{align*}
    \Delta \le \Sigma_{X} , &
\\
    \tr ( H_{j} \Delta H_{j}^{T} ) \le D_{j} - \tr ( \Sigma_{j} ) , &
    \quad \forall j \in \{ 0 , 1 , \cdots , k - 1 \} ,
\\
    \tr ( \Delta ) \le D_{X} . &
\end{align*}

